A geometric integration approach to smooth optimisation: Foundations of the discrete gradient method

Discrete gradient methods are geometric integration techniques that can preserve the dissipative structure of gradient flows. Due to the monotonic decay of the function values, they are well suited for general convex and nonconvex optimisation problems. Both zero- and first-order algorithms can be derived from the discrete gradient method by selecting different discrete gradients. In this paper, we present a thorough analysis of the discrete gradient method for optimisation which provides a solid theoretical foundation. We show that the discrete gradient method is well-posed by proving the existence of iterates for any positive time step, as well as uniqueness in some cases, and propose an efficient method for solving the associated discrete gradient equation. Moreover, we establish an $O(1/k)$ convergence rate for convex objectives and prove linear convergence if instead the Polyak-Lojasiewicz inequality is satisfied. The analysis is carried out for three discrete gradients-the Gonzalez discrete gradient, the mean value discrete gradient, and the Itoh-Abe discrete gradient, as well as for a randomised Itoh-Abe method. Our theoretical results are illustrated with a variety of numerical experiments, and we furthermore demonstrate that the methods are robust with respect to stiffness.

==> preamble.tex <==
\usepackage{commath} % Basic set notation
\usepackage{enumerate} % Enumerate environments
\usepackage{stmaryrd} % Further mathematical notations, such as \mapsfrom
\usepackage{xcolor}
\usepackage{textgreek} % for \textbeta etc
\usepackage{booktabs}
\RequirePackage[semicolon]{natbib}
\RequirePackage{graphicx}
\RequirePackage{amsthm}
\RequirePackage{amsmath}
\RequirePackage{caption}
\usepackage[hyphens]{url}
\usepackage{hyperref}
\hypersetup{
	colorlinks=true,
	breaklinks=true,
	filecolor=blue,
	urlcolor=blue,
	linkcolor=black,
	pdfpagemode=FullScreen,
	citecolor=blue
}

\makeatletter
\renewcommand\hyper@natlinkbreak[2]{#1}
\makeatother

\newcommand{\algoref}{Algorithm~\ref}
\newcommand{\condref}{Condition~\ref}
\newcommand{\corref}{Corollary~\ref}
\newcommand{\subsecref}{Subsection~\ref}
\renewcommand{\secref}{Section~\ref}
\newcommand{\tabref}{Table~\ref}
\newcommand{\inner}[1]{\langle#1\rangle}
\newcommand{\biginner}[1]{\left\langle#1\right\rangle}
\newcommand{\eps}{\varepsilon}
\newcommand{\CC}{\mathbb{C}} \newcommand{\EE}{\mathbb{E}}
\newcommand{\JJ}{\mathbb{J}} \newcommand{\KK}{\mathbb{K}}
\newcommand{\NN}{\mathbb{N}} \newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}} \newcommand{\RR}{\mathbb{R}}
\newcommand{\TT}{\mathbb{T}} \newcommand{\VV}{\mathbb{V}}
\newcommand{\ZZ}{\mathbb{Z}} \newcommand{\NNN}{\mathbb{N^*}}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\calA}{\mathcal{A}} \newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}} \newcommand{\calD}{\mathcal{D}}\newcommand{\calE}{\mathcal{E}} \newcommand{\calF}{\mathcal{F}} \newcommand{\calG}{\mathcal{G}} \newcommand{\calH}{\mathcal{H}} \newcommand{\calI}{\mathcal{I}} \newcommand{\calJ}{\mathcal{J}} \newcommand{\calL}{\mathcal{L}} \newcommand{\calM}{\mathcal{M}} \newcommand{\calN}{\mathcal{N}} \newcommand{\calO}{\mathcal{O}} \newcommand{\calP}{\mathcal{P}} \newcommand{\calQ}{\mathcal{Q}} \newcommand{\calR}{\mathcal{R}} \newcommand{\calS}{\mathcal{S}} \newcommand{\calT}{\mathcal{T}} \newcommand{\calU}{\mathcal{U}} \newcommand{\calV}{\mathcal{V}} \newcommand{\calX}{\mathcal{X}} \newcommand{\calY}{\mathcal{Y}} \newcommand{\calZ}{\mathcal{Z}}
\DeclareMathOperator{\BD}{BD}
\DeclareMathOperator{\BGV}{BGV}
\DeclareMathOperator{\BV}{BV}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\Co}{Co}
\DeclareMathOperator{\co}{co}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\ICTV}{ICTV}
\DeclareMathOperator{\Int}{int}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\Mod}{mod}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\TV}{TV}
\DeclareMathOperator{\TGV}{TGV}
\DeclareMathOperator{\SGN}{SGN}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\shrink}{shrink}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\SSIM}{SSIM}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Sum}{sum}
\DeclareMathOperator{\symm}{symm}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\theoremstyle{theorem}
\newtheorem{theorem}{Theorem}[section]%  meant for continuous numbers
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}%
\newtheorem{lemma}[theorem]{Lemma}%
\newtheorem{example}[theorem]{Example}%
\newtheorem{remark}[theorem]{Remark}%
\newtheorem{definition}{Definition}[theorem]

\numberwithin{equation}{section}

